A linear domain decomposition method for two-phase flow in porous media

This article is a follow up of our submitted paper [11] in which a decomposition of the Richards equation along two soil layers was discussed. A decomposed problem was formulated and a decoupling and linearisation technique was presented to solve the problem in each time step in a fixed point type iteration. This article extends these ideas to the case of two-phase in porous media and the convergence of the proposed domain decomposition method is rigorously shown.

==> praeambels_and_definitions/lualatexartikelpraeambel.tex <==
%Dies ist der Kopf meiner Skripte. Er enthaelt alle Pakete und Einstellungen

%%% BUG FIXING SECTION
% There ist a bug in thmtools. After Latex Upgrade change line 48 in thm-autoref.sty so that
% it reads
%\csname #2refname\@xa\endcsname\@xa{\thmt@envname}{#3}{#4}%
% then run texhash

%MAKROPAKETE
%1.PAKETE DIE MIT DER KODIERUNG VON ZEICHEN ZU TUN HABEN.
%\usepackage[german]{babel}
%Definition von Sprachabhaengigen Komponenten insbesondere fuer Dokumente
%in anderen Sprachen als Englisch
\usepackage{fixltx2e}
\usepackage{etex} %some fix for hyperref
%Korrektur einiger Fehler die sich in LaTeX2e eingeschlichen haben. 
%\usepackage{ngerman} 
% stellt Sonderzeichen und ihre Befehle wie zum Beispiel "o zur Verfuegung

%%%%%%%%%%%% SCHRIFTEN %%%%%%%%%%%%%%%%%%%%%%%%
%\usepackage{mathpazo}%andere Schriftart
%\usepackage{lmodern}
%\usepackage{beramono}
% Using Courier font
\renewcommand{\ttdefault}{pcr}
%Tweak, damit auch im Mathemodus tt-schrift fettgedruckt werden kann.

%%%% PDFLaTeX or LUALaTeX %%%%%%%
%% if pdflatex is used uncomment the following packages. If lualatex is used comment them.
%dieses Paket ermoeglicht die Eingabe von Sonderzeichen ueber die Tastatur
% \usepackage[utf8]{inputenx}
% %additions for utf8
% \input{ix-utf8enc.dfu}
%% comment \usepackage{uiinput} if lulatex is used! line 131
%% if pdflatex is used uncomment above packages. If lualatex is used comment them.
\usepackage{microtype}
\usepackage[dvipsnames,svgnames,table]{xcolor} % Farben

\usepackage[T1]{fontenc} %Kodierung von Zeichensaetzen. 
	%Das optionale Argument <Kodierung> kann eine durch Komma getrennte Liste von
%Kodierungen enthalten. Im Text koennte dann an %beliebiger %Stelle zum wechseln der
%Kodierung die Befehlsfolge:
    		%\fontencoding{<Kodierung>}
    		%\selectfont
	%verwendet werden. Gaengige Kodierungen sind:
%                           Tabelle 5.4: Kodierungen
%         T1      8-Bit-Standard fuer EC-Fonts	 
%         TS      8-Bit-Zeichenkodierung fuer TS-Fonts
%         OT1      7-Bit-Kodierung fuer Text1 , CM-Fonts
%         OML      7-Bit-Kodierung fuer Formeltext1
%         OMS      7-Bit-Kodierung fuer mathematische Symbole1
%         OMX      7-Bit-Kodierung fuer erweiterte mathematische Symbole1
\usepackage{latexsym}
%Definiert zusaetzliche Symbolbefehle.
\usepackage[full]{textcomp}
% Sammlung von Textsymbolen. Optional kann [safe] oder [full]
% als Option hinzugefuegt werden, lezteres aber nur bei
%CM und EC-Fonts

\usepackage{eucal}
%Stellt deutsche Frakturschrift im Math Modus zur Verfuegung bei \mathcal
%\usepackage{sistyle,upgreek}
%\usepackage{fixmath}
% sistyle stellt \SI{Masszahl}{Einheit}
% bereit, zur si-konformen Darstellung von phy Goessen. textcom und upgreek stellt
% fweiter Symbole bereit, welche sistyle braucht. Ausserdem diese Befehle \micro,
% \ohm, \SIdecimalsign{,}(legt die trennung bei Dezimalzahlen fest)
% \SIproductsign{\cdot} (legt das Multiplikationszeichen fest) \SIgroupfourfalse
% erzeugt bei grossen Zahlen kleine Abstaende zwischen 3ergruppen \ang{zahl} ist das
% gradzeichen.
\usepackage{mathrsfs} %Stellt schreibschrift zur verfuegung im Mathemoduns mit \mathscr

%1.01 LAYOUTPAKETE
\usepackage[left = 2.5 cm, right = 2.5 cm, top = 2.5 cm, bottom = 3cm]{geometry} %a4paper
% left = 3.5 cm, right = 3.5 cm, top = 3.3 cm, bottom = 6.6cm
%\usepackage{fancyhdr}%Wird fuer erweiterte Kopf- und Fusszeileneinstellungen benoetigt.

%\usepackage{enumerate}%Stellt die freie Auswahl von Aufzaehlungszeichen zur Verfuegung
\usepackage[shortlabels]{enumitem} %Anpassbare Enumerates/Itemizes mit [label=]
									%shortlabels: komp.  zu enumerate
%Packete zur benutzung des KOMA-Paketes fuer europaeische Layouts also zur
%Benutzung von 'scrartcl' fuer Artikel, 'scrreprt' fuer umfangreiche %Artikel und
%Artikelsammlungen, 'scrbook' fuer Buecher und %'scrlettr2' fuer Briefe:
%\usepackage{scrpage2} %fuer Kopf- und Fusszeilen, 
%\usepackage{scrdate,scrtime}% fuer Wochentag und Uhrzeit, 
%\usepackage{scraddr}
%zur Loesung von Problemen mit Paketabhaengigkeiten scrfile sowie fuer
%Briefadressverwaltung scraddr. 

%%%% neue Befehle
%Zahlensymbole

%1.1PAKETE NOTWENDIG FUER MATHEMATISCHE FORMELN 
\usepackage{amsfonts}%Fonts = Schriftarten der American mathematical Society (ams)
\usepackage{amssymb}%Mathematische Symbole der ams.
\usepackage{bbm}
\usepackage{amsmath} 
%Definiert viele weitere Befehle fuer mathematischen Formeln und darueber hinaus.
\usepackage{exscale}
% Skaliert mathematische Symbole in anderen Schriftarten als ‚cmex10‘, so dass
% falls die Schriftart in anderen Groessen als 10pt vorliegt diese angepasst
% werden koennen
\usepackage{amstext}
% erlaubt es in abgesetzten Gleichungen mit \text kurzen Text einzufuegen.
%\usepackage{amsextra}%hauptsaechlich fuer die Kompatibilitaet von Dokumenten
%gebraucht.
%\usepackage[arrow,matrix,curve]{xy} 
% Packet xy-pic um Kommutative Diagramme und
% zweidim Zeichnungen zu %zeichnen.in den eckigen Klammern stehen Module die
% geladen werden, je nach dem was man braucht. In der %Matheumgebung wird das so
% benutzt: \begin{xy} ...\end{xy}

%Theoremumgebungen
\usepackage{amsthm}%Ermoeglicht kontrolle ueber die Theorem-Umgebung beisst
%sich mit ntheorem funktioniert aber mit \usepackage{thmtools}
\usepackage{thm-patch,aliasctr,parseargs,keyval}
\usepackage{thmtools}
%stellt \declaretheorem[style=definition,qed=$\rtimes$]{definition}
%zur verfuegung
% There ist a bug in thmtools. After Latex Upgrade change line 48 in thm-autoref.sty so that
% it reads
% \csname #2refname\@xa\endcsname\@xa{\thmt@envname}{#3}{#4}%
% then run texhash

%Erlaubt das Setzen fetter Symbole mit \boldymbol{} bzw\pmb{}
\usepackage{bm} 
\usepackage{amsbsy}
% stellt die Befehle \bm \hm zur Verfuegung, um mathematische
% Symbole fett zu machen. Muss nach allen Fontpacketen geladen %werden!!!

% if LUALaTeX is used uncomment this
%\usepackage{uniinput} %ermoeglicht die Eingabe von unicode Zeichen


%\usepackage{listings} 
%Wird verwendet um sourcecode zu TeXen, stellt 
%\begin{lstlisting} .. \end{lstlisting} und \lstinputlisting zur Verfuegung
                                                                   
 
%2.PAKETE FUER GRAFIKEN UND GLEITOBJEKTE
\usepackage{float,scrhack}
%Stellt zusaetzliche Befehle fuer Gleitobjekte zur Verfuegung
\usepackage{wrapfig}
%Stellt die Moeglichkeit zur Verfuegung Text um Bilder herumlaufen zu lassen.
\usepackage[textfont=it,labelfont=bf,format=plain]{caption}
% Ermoeglicht das einstellen von figureumgebungen
\usepackage{subcaption}

\usepackage{array}%Verbessert die Darstellung von Tabellen und stellt erweiterte Befehle
%zur Verfuegung.
\usepackage{hhline} %stellt den \hhline in Tabellen zur Verfuegung
\usepackage{delarray}
%stellt eine einfachere Umgebung fuer begrenzte Arrays zur
%Verfuegung.\begin{array} LB {<Spaltenvereinbarung>} RB

% das tabu Packet, ein machtiges Tabellenpaket
\usepackage{tabu}
\usepackage{colortbl} % Farben in Tabellenzeilen

%\usepackage{flafter} %Verhindert, dass Gleitobjekte in einem Dokument vor die
%Stelle gesetzt werden, an der sie in der Eingabedatei %aufgebaut werden.
%\usepackage{graphpap}%Zum Setzen von „Millimeter“-Papier. Es definiert den
%graphics paper-Befehl in der picture-Umgebung. 

%\usepackage[]{graphicx} %vorsicht, laedt hyperref
%\usepackage{sidecap}
%Für das malen von Graphen
%Für das malen von Grafiken
% waehle zunaechst das richtige Treiberbackend fuer Tikz.
% beamer erkennt z. T nicht das richtige backend. pgfsys-pdf.def ist die Option, die am meisten unterstuetzt.
%Für das malen von Graphen
\usepackage{tikz}
\usepackage{pgfplots}
\pgfplotsset{compat=newest}
\usetikzlibrary{arrows,%
%                 petri,%
%                topaths,%
%		fit,%
%		positioning,%
%		decorations.pathmorphing,%
%		backgrounds,%
}%

% Ausgabe von Grafiken als externe Grafik
\usetikzlibrary{external}
% \usepgfplotslibrary{external}
\tikzset{external/optimize=true}%
% \tikzset{external/system call= {pdflatex -enable-write18 -shell-escape %
% % % 				  -save-size=80000 %
% % %                                -pool-size=100000000 %
% % %                                -extra-mem-top=500000000 %
% % %                                -extra-mem-bot=100000000 %
% % %                                -main-memory=900000000 %
%                                \tikzexternalcheckshellescape %
%                                -halt-on-error %
%                                -interaction=batchmode %
%                                -jobname "\image" "\texsource"}} 
\tikzexternalize[%
% %mode=graphics if exists,
  up to date check=md5,
 figure list=true,
 prefix=Tikzcache/,%
 ]
\tikzifexternalizing{%
% don’t include package XYZ here
}{%
%hier kommen Pakete hinzu, die Probleme mit der external library von tikz haben
%\usepackage{pdfpages}
%\usepackage{vmargin}
% this package is incompatible with tikz externalization and is problematic
}%
% \usepackage[textsize=normal,textwidth=2cm,obeyFinal]{todonotes}
% %obeyDraft lässt die Notes erscheinen, wenn man draft an hat und nicht, wenn nicht. Vertraegt sich nicht mit hyperref

% % additional todo stuff
% % extra functionality for todonotes taken from the manual
% % usage: \mycomment[HSM]{Testing second time.}.
% \newcounter{mycomment}
% \newcommand{\mycomment}[2][]{%
% % initials of the author (optional) + note in the margin
% \refstepcounter{mycomment}%
% {%
%   \setstretch{0.7}% spacing
%   \todo[color={red!100!green!33},size=\small]{%
%   \textbf{Comment [\uppercase{#1}\themycomment]:}~#2}%
% }}
% 
% % mark whole section
% \newcommand\todoin[2][]{\todo[color={green},inline, caption={2do}, #1]{
% \begin{minipage}{\textwidth-4pt}#2\end{minipage}}}
% % This example renders like
% % \todoin{
% % 	Some text.
% % 	\begin{align}
% % 	\sin(\theta)^2 + \cos(\theta)^2 = 1
% % 	\end{align}
% % 	A formula and a list
% % 	\begin{itemize}
% % 		\item An item
% % 	\end{itemize}
% % }
% 
% % numbered todonotes 
% \newcommand{\ntodo}[2][]{\todo[#1]{\thesubsection{}. #2}}
% % combining everything
% \newcounter{todoListItems}
% \newcommand{\sstodo}[2][]
% {\addtocounter{todoListItems}{1}
% \todo[caption={\protect\hypertarget{todo\thetodoListItems}{}\thesection. #2}, #1]
% {\begin{spacing}{1} \hfill \hyperlink{todo\thetodoListItems}{#2} \end{spacing} }}


%\usepackage[position=top]{subfig}
% BIBLIOGRAPHIE 
\usepackage[
	  backend=biber,
%	  bibliographystyle=alphabetic,
%	  style=ieee,		%globaler Style (Zitier- und Bibstil)
	  citestyle=numeric, 	% Zitierstil
%	  bibliographystyle=chem-acs,	% Bibliographiestil
	  firstinits=true, 		% Vornamen abruerzen
	  sorting=nty, %sort by name,title,year
	  maxbibnames=99,
%         maxnames=99,
          language=british,
%          abbreviate=true,
	  doi=false,
          isbn=false,
          url=false,
          sortcites=true,
          backref=true,
          defernumbers=true,
]{biblatex}
\addbibresource{/home/seusdd/Dissertation/Bibliographie/dissertationsliteratur.bib}


%3.PAKETE, DIE DAS ERSTELLEN EINES INDEX ERLEICHTERN
%\usepackage{makeidx} 
%'makeidx' Stellt Befehle fuer Indexerstellung zur Verfuegung.
%\usepackage{showidx}%'showidx'bewirkt die Anzeige von Indexeintraegen %im
%Randbereich.

%3.SONSTIGE NUETZLICHE PAKETE
%\usepackage{ifthen}%Definiert einfache Strukturen der Programmiersprachen
%\usepackage{alltt} % verbatim-Umgebung mit Interpretation von Befehlen.
%Analysepaket zur ueberpruefung der Korrektheit der Syntax bei unterdrueckter
%Ausgabe:
%\usepackage{syntonly}% stellt dem Anwender den Befehl '\syntaxonly'zur Verfuegung,
%der in der Praeambel angegeben werden muss, um beim
%Formatieren die Ausgabe zu unterdruecken; eine bereits vorhandene .dvi-Datei
%bleibt also erhalten.


%%%% REFERENZIERUNG %%%%% 
% Die Reihenfolge der folgenden 4 Packete ist wichtig.
\usepackage{nameref}
\usepackage[english]{varioref}%Stellt erweiterte Befehle zur Referenzierung von
%Gleitobjekten zur Verfuegung
\usepackage[citecolor=black,urlcolor=blue,linkcolor=blue,colorlinks=true,pdfborder={0 0 %
0},pdfpagelabels,plainpages=false,naturalnames,unicode]{hyperref}
\usepackage{memhfixc}
%\usepackage[ngerman,capitalize]{cleveref}
\usepackage[]{cleveref}

\usepackage{bookmark}
% Fix fuer das referenzieren von figures
%\usepackage[all]{hypcap}


%SEITENEINSTELLUNGEN
\setlength{\parindent}{0cm} %Hebt die Einrueckung von Absaetzen auf.
%\setlength{\textwidth}{14.5cm} %Legt die Textbreite fest
\pagestyle{myheadings} 
%\usepackage{titlepage}

%'plain' wuerde den Seitenkopf leer lassen aber die Seiten unten
%mittig durchnummerieren. 'empty' laesst die Seite komplett leer
%\markright{\today\hfill}
%\usepackage{changepage}
\allowdisplaybreaks[1] %Erlaubt bei der Align-Umgebung dass Zeilen auf
%verschiedene Seiten gesetzt werden. die zahlen 1-4 koennen angegeben werden um
%das Umbrechen noch weiter zu forcieren.

%\pagestyle{fancy}  \fancyhf{}  
%\renewcommand{\headrulewidth}{0.4 pt}%Strichdicke  
%\setlength{\headheight}{1.2 cm}%Hoehe der Kopfzeile
 
%\fancyhead[EL]{\page}
%\fancyhead[ER]{\textsc{\rightmark}}
%\fancyhead[C]{{\Large \textbf{FK019 freier Fall, g-Leiter}}\\\small 24.10.2008}
%\fancyhead[OR]{\page}
%\fancyhead[OL]{\textsc{\rightmark}}

%% todo makros

% self made todo solution
\newcommand{\todo}[1]{\marginpar{\textcolor{red}{[\textbf{TODO:} #1]}}}
\newcommand{\todox}[1]{\textcolor{red}{[\textbf{TODO:} #1]}} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

